Neural Distributed Source Coding

Distributed source coding (DSC) is the task of encoding an input in the absence of correlated side information that is only available to the decoder. Remarkably, Slepian and Wolf showed in 1973 that an encoder without access to the side information can asymptotically achieve the same compression rate as when the side information is available to it. While there is vast prior work on this topic, practical DSC has been limited to synthetic datasets and specific correlation structures. Here we present a framework for lossy DSC that is agnostic to the correlation structure and can scale to high dimensions. Rather than relying on hand-crafted source modeling, our method utilizes a conditional Vector-Quantized Variational Autoencoder (VQ-VAE) to learn the distributed encoder and decoder. We evaluate our method on multiple datasets and show that our method can handle complex correlations and achieves state-of-the-art PSNR. Our code is made available at https://github.com/acnagle/neural-dsc.

==> figures/fig_discus.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=12cm]{images/discus_parallel.png} % draft
\caption{DISCUS  }\label{fig:discus} % bold and font - need some work. Is this figure useful? 
\end{figure}



==> figures/fig_dist_vs_separate_reconst.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{images/dist_vs_separate_reconst.pdf}
\vspace{-0.3em}
\caption{\footnotesize Reconstructions of test set images using distributed vs. separate encoders.  The dimmed portion in the ground truth is used as side information to compress the top half of the image.  As readily visible in the figure, the distributed encoder preserves the details and overall color more faithfully than the separate encoder.}
\label{fig:fig_dist_vs_separate_reconst}
\end{figure}

==> figures/fig_dist_vs_side.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=12cm]{images/dist_vs_side4.png} % draft
\caption{Coding with side information available at the decoder (left) and both the encoder and decoder (right). An encoder that has no access to the correlated side-information can asymptotically achieve the same compression rate as when side-information is available at both the encoder and the decoder.  }\label{fig:dist-vs-side}
\end{figure}


==> figures/fig_drasic.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=0.9\linewidth]{images/DRASIC.png} % m -> m_1
\caption{DRASIC empirically shows that the recurrent autoencoder-based compression for separate encoders (middle) and common encoders (left) are comparable as long as the decoders are common~\cite{DRASIC2020}. DRASIC is }\label{fig:drasic} 

\end{figure}



==> figures/fig_drasic_vs_ours.tex <==
\begin{figure}[!h]
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=0.7\linewidth]{images/diagram_drasic.pdf}
  \vspace{-0.3em}
  \caption{Individual Encoders, \textit{Shared} Decoder (DRASIC)}
  \label{fig:diagram_drasic}
\end{subfigure}
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=0.7\linewidth]{images/diagram_ours.pdf}
  \vspace{-0.3em}
  \caption{Individual Encoders, \textit{Joint} Decoder (this paper)}
  \label{fig:diagram_ours}
\end{subfigure}
\vspace{-0.5em}
\caption{\footnotesize (top) Diagram showing the shared decoder scheme used by DRASIC \cite{DRASIC2020}. (bottom) Diagram showing the \textit{joint} decoder scheme used in this paper.}
\label{fig:drasic_vs_ours}
\end{figure}


==> figures/fig_gaussian_rate_dist.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.9\linewidth]{images/gaussian_rate_dist.pdf}
\vspace{-0.5em}
\caption{\footnotesize Rate-distortion points of learned joint and distributed encoders compared to theoretically best compressors. The ``Optimal'' curves represent the asymptotically optimal rate-distortion points and are included as reference.  Note that these are theoretical limits and do not correspond to any concrete compression scheme.}
\label{fig:gaussian_rate_dist}
\vspace{-0.5em}
\end{figure}

==> figures/fig_grad_full_comparisons.tex <==
\begin{figure}[htbp]
\centering
  \centering
  \includegraphics[width=0.9\linewidth]{images/mnist_grad_epoch_test_acc.pdf}
  %\caption{}
  \label{fig:grad_comparison_test_acc}
% \begin{subfigure}{.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/mnist_grad_epoch_train_loss.pdf}
%   %\caption{}
%   \label{fig:grad_comparison_train_loss}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.49\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/mnist_grad_epoch_test_acc.pdf}
%   %\caption{}
%   \label{fig:grad_comparison_test_acc}
% \end{subfigure}
\vspace*{-0.5 em}
\caption{\footnotesize Distributed training performance with compressed gradients using a distributed encoder in comparison to other baseline methods in terms of test set accuracy.  Note that standard error is very small and barely visible, and may require zooming in on an electronic copy of this manuscript.}
\label{fig:grad_full_comparisons}
\end{figure}


==> figures/fig_grad_rate_distortion.tex <==
\begin{figure}[htbp]
\centering
% \includegraphics[width=0.9\linewidth]{images/mnist_grad_train_loss.pdf}
\includegraphics[width=\linewidth]{images/mnist_grad_test_acc.pdf}
\caption{\footnotesize Plot of the average test set accuracy over the course of training $\net$ using compressed gradients. We observe that the distributed encoder leads to comparable accuracy as the joint encoder, but using about only half of the communication cost. Shaded regions represent standard error.
}
\label{fig:grad_performance}
\end{figure}


==> figures/fig_grad_vqvae_mse.tex <==
% \begin{figure}[h]
% \centering
% \begin{subfigure}{.8\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/mnist_grad_vqvae_train_mse.pdf}
%   % \caption{}
%   \label{fig:grad_vqvae_mse_train}
% \end{subfigure}

% \begin{subfigure}{.8\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/mnist_grad_vqvae_val_mse.pdf}
%   % \caption{}
%   \label{fig:grad_vqvae_mse_val}
% \end{subfigure}
% \vspace*{-4mm}
% \caption{\footnotesize Average $\ell_2$ distortion over training (left) and validation (right) sets during the course of VQ-VAE training.  We clearly see that the distributed encoder significantly outperforms the separate encoder and approaches the distortion of the joint encoder.}
% \label{fig:grad_vqvae_mse}
% \end{figure}


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.9\linewidth]{images/mnist_grad_vqvae_val_mse.pdf}
  \caption{\footnotesize Average $\ell_2$ distortion over the validation split during the course of VQ-VAE training.  We observe that the distributed encoder significantly outperforms the separate encoder and approaches the distortion of the joint encoder.}
\label{fig:grad_vqvae_mse}
\end{figure}

==> figures/fig_jds_settings.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.7\linewidth]{images/jds_settings.pdf}
\vspace{-0.5em}
\caption{\footnotesize Joint encoder (top): $\msg = f(\orig;\sinfo)$, $\hat{\orig} = \fdecode(\msg;\sinfo)$.
Distributed encoder (middle): $\msg = f(\orig)$, $\hat{\orig} = g(\msg;\sinfo)$.
Separate encoder (bottom): $\msg = \fencode(\orig)$, $\hat{\orig} = \fdecode(\msg)$. }
\label{fig:jds_settings}
\vspace{-0.5em}
\end{figure}

==> figures/fig_kitti_bpp_psnr.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.9\linewidth]{images/fig_kitti_stereo_bpp_psnr2.pdf}
\vspace{-0.5em}
\caption{\footnotesize Comparison of rate-distortion curves on the KITTI Stereo image dataset. Our method achieves higher PSNR than other methods for low rates and remains competitive for higher rates.}
\label{fig:kitti_bpp_psnr}
\vspace{-0.5em}
\end{figure}


==> figures/fig_placeholder.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=10cm,height=4cm]{images/placeholder.png}
\caption{Placeholder caption.}
\label{fig:placeholder}
\end{figure}

==> figures/fig_slepianwolf.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=8cm]{images/slepianwolf.jpg} % draft
\includegraphics[width=5cm]{images/dist_vs_side2.jpg} 
\caption{Left: distributed compression system. Middle: Optimal rate region for lossless compression (Slepian-Wolf theorem; shade will be added); Right (bubble): Coding with side information available only to the decoder}\label{fig:slepian-wolf} % Typo H(y|x) in the right figure. 
\end{figure}

